Unleashing the Power of Meta-tuning for Few-shot Generalization Through Sparse Interpolated Experts

Recent successes suggest that parameter-efficient fine-tuning of foundation models as the state-of-the-art method for transfer learning in vision, replacing the rich literature of alternatives such as meta-learning. In trying to harness the best of both worlds, meta-tuning introduces a subsequent optimization stage of foundation models but has so far only shown limited success and crucially tends to underperform on out-of-distribution (OOD) tasks. In this paper, we introduce Sparse MetA-Tuning (SMAT), a method inspired by sparse mixture-of-experts approaches and trained to isolate subsets of pre-trained parameters automatically for meta-tuning on each task. SMAT successfully overcomes OOD sensitivity and delivers on the promise of enhancing the transfer abilities of vision foundation models beyond parameter-efficient fine-tuning. We establish new state-of-the-art results on a challenging combination of Meta-Dataset augmented with additional OOD tasks in both zero-shot and gradient-based adaptation settings. In addition, we provide a thorough analysis of the superiority of learned over hand-designed sparsity patterns for sparse expert methods and the pivotal importance of the sparsity level in balancing between in-distribution and out-of-distribution generalization. Our code is publicly available.

==> sections/iclr_instructions.tex <==

\section{Submission of conference papers to ICLR 2024}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2024 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2024_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2024_conference.sty+ and \verb+iclr2024_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2024_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/method.tex <==
\section{SMAT: Sparse MetA-Tuning}
%We begin with a motivating example in \cref{sec: motivating_example} which lead to our proposed meat-tuning method in \cref{sec: mt_train}. Lastly, we propose a gradient-free meta-test time adaptation algorithm tailored for our proposed method in \cref{sec: mt_adapt}.


{\color{blue} Jihoon's overall comment on the method part}

\chen{I am re-writhing this section in the method\_v2.tex file}.


\js{Unfortunately this overall section is quite messy and states a lot of things without really telling a story. Why are these choices made? What's the motivating principle? What problem is this solving? Why is it clever?}
\subsection{Sparse modulations of a pre-trained model finds generalizable skills} \label{sec: motivating_example}
%%%%%%%%%%%%%%%%%%%%TODOS:%%%%%%%%%%%%%%%%%%%%%%%%%%
% complete figures or tables
% list all the details
% consider move to the appendix and leave only important and precise description and findings here
%%%%%%%%%%%%%%%%%%%%TODOS:%%%%%%%%%%%%%%%%%%%%%%%%%%

\js{I like the idea of starting with a motivating example, but at the moment this makes for a rather abrupt transition that is difficult to follow. Explain first what you are trying to show before diving into details.}
\textbf{A motivating example.}$\ \ $To motivate our method, we select one domain as an ID source for meta-training, and one domain as OOD for meta-testing to measure generalizability, from DomainNet~\cite{peng2019moment}. For meta-training, we meta-train the model initialized with $\theta_{pre}$, using ProtoNet~\cite{snell_prototypical_2017}, on ID few-shot tasks to obtain $\theta_{mt}$, the meta-tuned model. For meta-testing on each one of the five OOD domains, we first optimize a set of binary masks\js{how?} $\boldsymbol{z}\in\{0,1\}^{|\theta_{mt}|}$ on tasks from the training split which results in a sparse binary interpolation $\tilde{\theta}_{domain}$ between $\theta_{mt}$ and $\theta_{pre}$, that is
\begin{equation}
    \theta_{domain} = \boldsymbol{z}_{domain}\odot(\theta_{mt}-\theta_{pre}) + \theta_{pre}.
\end{equation}
We define $\theta_{mt}-\theta_{pre}$ as the \textbf{modulation}, thus $\boldsymbol{z}\cdot(\theta_{mt}-\theta_{pre})$ the \textbf{sparse modulation}, on $\theta_{pre}$.
%we select one domain (e.g., painting) as the meta-training domain out of the 6 available domains in the DomainNet~\cite{}dataset, and meta-train a model initialized from a pre-trained checkpoint $\theta_{pre}$ on 5-way-1-shot tasks sampled from its training split to obtain $\theta_{painting}$. Next, for each one of the remaining 5 OOD domains, we optimize a set of mask in binary space $\mathcal{M}\in\{0,1\}^{|\theta|}$ on its training tasks.
%The resultant model $\tilde{\theta}_{domain}$ is effectively a binary interpolation between the two pre-trained and ID meta-trained models. \par
%We use sigmoid as a soft approximation to binary values for $\mathcal{M}$ to enable gradient-based optimization. To ensure the final masks are binary, we use a very large learning rate of $1e^7$ and round the mask to $0/1$ before testing. 
\par
\textbf{Key takeaways.}$\ \ $Fig.~\cite{fig:X} depicts the meta-testing results of these $\theta_{domain}$ on all six domains. We highlight our findings: Despite neither $\theta_{pre}$ nor $\theta_{mt}$ having been trained on the OOD tasks, we make two important observations. \textbf{(a)} There exists a sparse modulation that results in better OOD generalization on that domain relative to using $\theta_{pre}$ and $\theta_{mt}$ directly.
%despite the two checkpoints have never been trained on the OOD testing domains. 
\textbf{(b)}, by merging a manually selected subset of masks (through their element-wise union) the resultant model, $\theta_{\delta}\cdot\cup\boldsymbol{z}$ can achieve comparable, if not, better performance relative to both $\theta_{pre}$ and $\theta_{mt}$ on all ID and OOD domains.\par

This suggests that an optimal point can be found which has preferable trade-offs between the two sets of parameters. In the following paragraphs, we describe a section that motivates this idea.

% \textbf{Discussion: Why dense training fails to reach the merged solution all in once.}

\subsection{Meta-learning sparse modulation with controlled $\textit{L}_0$ Sparsity} \label{sec: mt_train}
% give a quick overview here
\textbf{Method overview.}$\ \ $
%Our observations essentially suggest sparsification in modulation parameters and selectively merging a subset of them in a task-dependent manner are the keys to attain good ID and OOD generalization.
To this end, we propose Spare MetA Tuning (\textbf{SMAT}). The central idea of SMAT is to enforce the sparsity of the modulation (i.e., adapted weights from the pre-trained model; $\theta_{\mathtt{mt}}-\theta_{\mathtt{pre}}$), and selectively merging the sparse modulations to improve both ID and OOD generalization by meta-learning a task-dependent merging strategy. As illustrated in Fig.~\ref{fig:overview}, SMAT integrates three essential elements into a single round of end-to-end meta-tuning: \textbf{(a)} automatic discovery of a set of sparse masks and a shared dense modulation through controlled sparsity constraints, which jointly define the set of distinct sparse modulation; \textbf{(b)} meta-learning a hypernetwork for task-dependent mask selection, hence achieve task-specific inference with the merged model $\boldsymbol{\theta}_i$ through a systematic merging operation defined by $\boldsymbol{\theta}_i = \boldsymbol{\theta}_{pre} +  \boldsymbol{\theta}_{\delta}\odot\sum_{m}^{|\gM|}\alpha_{i,m}\boldsymbol{z}_m$; \js{Should this be a union? Otherwise you might have values larger than 1} and \textbf{(c)}, a bootstrapping strategy with a dense target model to further encourage knowledge transfer and mask specialization.










% Although the example also illustrate that the merged solution lies in the hypothesis space of approaches that simply meta-tuning the entire pre-trained model, the reasons why naively meta-training $\theta_{pre}$ on the ID tasks cannot recover the final merge solution is primarily due to the lack of mechanisms during meta-training that explicitly encourage specialization and cooperation. To this end, we propose our solution: {\sc SMAT}. %We hypothesize that systematic generalization across both ID and OOD testing tasks can be achieved by appropriately select and merge a subset of common sparse modulations according to a pre-defined merging operation, e.g., union. 

% As illustrated in Fig.~\ref{fig:overview}, our approach integrates the following two essential elements into a single round of end-to-end meta-tuning: (a) automatic discovery of a fixed set of binary masks and a shared dense modulation through controlled sparsity constraints, which jointly defines the set of sparse modulation; and (b) meta-learning a hypernetwork for task-dependent mask selection, hence achieve task-specific inference, through a systematic merging operation

% define modulation as $\theta_i - \theta_{pre}$, i.e., the difference between the pre-trained and meta-tuned model parameters.\par
% We assume the ID and potentially many of the unseen OOD tasks share a set of common skills. To this end , we propose SMAT a meta-learning algorithm that automatically discover a diverse skill sets on IID tasks through sparsity regularization, and meta-learn a simple combination rule in the form of a hypernetwork.\par

%We resort to sparsity for combating the redundancy in large pre-trained models and during meta-training. As the pre-trained model is already powerful, %intuiatively it should only require small local update rather than full-fine-tuning for it to acquire few-shot learning skills.  We resort to spasrity to %overcome the redudancy in the model parameters during meta-tuning. Besides, spassity identifies a tiny subset of parameters which are belived to be more %specialzied and essential. With sparsity leel being.

\textbf{Sparsification.}$\ \ $As evident in~\cref{sec: motivating_example}, distinct sparse modulation that achieves effective generalization performance can co-exist on a common set of dense modulation parameters, $\boldsymbol{\theta}_{\delta}=\boldsymbol{\theta}_{pre}-\boldsymbol{\theta}_{mt}$; therefore, we induce the $m$-th sparse modulation in the form of a sparse reparameterization $\boldsymbol{\theta}_{\delta}\odot\mathbf{z}_m$, associated with the $m$-th binary mask $\boldsymbol{z}_m \in \gM$, of a \textit{common} dense modulation $\theta_{\delta}$ shared by all $|\gM|$ different masks. To this end, sparsification is achieved by imposing sparsity constraints on the binary masks, $\boldsymbol{z}_m\in\gM$. We let the total number of masks $|\gM|$ be a hyperparameter. To learn discrete binary masks through gradient-based optimization, we take inspiration from MSCN~\citep{schwarz2022meta}, and reparameterize the $m$-th binary masks with an underlying continuous distribution $q_{\phi_m}$ with with parameters $\phi_m$. The reparameterization samples i.e., $\mathbf{s}_m\sim q_{\phi_m}(\mathbf{s})$, can be transformed to have values \emph{exactly} $0$ and $1$ through a hard rectification $\mathbf{z}_m = g(s_m):=\min(1, \max(0, s_m))$. As a result, sparsity in masks can be enforced by limiting the probability of $s_m$ being non-zero which translates to limiting $1-Q_{\phi_m}(s\leq0)$ of $q_{\phi_m}$, where $Q$ is the CDF.  Choosing $q_{\phi_m}$ as the stretched hard concrete distribution~\citep{louizos2018learning} enables both reparameterization sampling and evaluation of the CDF analytically.\par

%The final sparsity constraint is imposed on the expected task-specific sparsity over all meta-tuning tasks to avoid the need for task-specific Lagrangian multiplier as we reformulate Eqn~(\ref{eq:sparsity_constraint_op}) into an unconstrained min-max game in the next section.

% Beside, we advaote for sparsity regualrization due to less interfernce thereby poteitnlaly improv. Many works have previously found the redundency in the saprsity apptern of large pre-trained languate or vision models.
% Learning a sparse pattern 

% Adapting a hand-crafted subset of parameters from a pre-trained or meta-learned initialization has shown potential to improve generalization performance of the task-specific model over adapting the entire model~\citep{shysheya2023fit}. Manually selecting a fixed set of parameters in the inner-loop or (and) outer-loop for adaptation, however, introduces strong bias which may be sub-optimal for the tasks of interest. Some prior works have advocated for formulating learning where to update in the model as a meta-learning problem~\citep{lee2018gradient,von2021learning}, leading to automatic discovery of patterned sparsity in the inner-loop update rule through meta-training. Nevertheless, these approaches still suffers from overwriting the pre-trained information by having a dense outer-loop parameter update in the full pre-trained parameter space. 
% % We seek a method that


% We hypothesis (evidence) that the effective skill acquisition for each task can be achieved by selectively updating a critical subset of parameters in a pre-trained model. These parameters are inherently task-specific. To this end, we propose 
% % MSCN(\chen{temp name}) 
% Sparse MetA-Tuning (SMAT)
% which given a pre-trained model $\boldsymbol{\theta}_{pre}$, meta-learns initialization for both a sparse binary mask $\mathbf{z}_0$ along with an associated set of dense modulation parameters $\boldsymbol{\zeta_0}$. 

% such that adapting the two jointly through a few inner-loop optimization steps yields a sparse, task-specific, elementwise product $\boldsymbol{\zeta}_K\odot\mathbf{z}_K$ that can be stitched to the original pre-trained initialization, i.e., $\boldsymbol{\theta}_{task} = \boldsymbol{\theta}_{pre} + \boldsymbol{\zeta}_K\odot\mathbf{z}_K$ to achieve good task-specific generalization. Such embarrassingly simple approach sufficiently addresses both 1) fast task-specific adaptation by meta-learning a separate modulation initialization 2) preserves transferable pre-trained information by imposing sparsity constraint on the mask $\mathbf{z}$. We now describe our meta-training optimization procedure for discovering such mask and modulation parameters. 

% \textbf{Reduce Distortion through Model Stitching.}$\ \ $ The introduced sparse modulation $\boldsymbol{\zeta}\odot\mathbf{z}$ allows for a straight-forward way to exploit a pre-trained model initialization; we simply "stitch" the sparse modulation to the pre-trained initialization which reminiscent a dense model ensemble in the weight space.
% However, naively stitching the final task-specific model raise concerns on 1) the compatibility issues, as this may be suboptimal task-specific solution 2) the pre-trained information is not exploited during training which could in turn affect both the expressiveness and quality of the learned sparse modulation. We propose to resolve both issues by simply involving $\theta_0$ in the meta-training objectives which results in the following meta-objectives:
% \begin{align}\label{eq:sparsity_uncon_op}
%        & \boldsymbol{\phi}_0^*,\boldsymbol{\zeta}_0^*,\lambda^* \doteq \argmin_{\boldsymbol{\phi}_0,\boldsymbol{\zeta}_0} \argmax_{\lambda\geq0} \mathcal{L}_{\mathcal{T}_i^q}(f_{\boldsymbol{\theta}_0 + \boldsymbol{\zeta}_K\odot\mathbf{z}_K}) + \frac{\lambda}{\text{\small dim}(\boldsymbol{\phi})}\sum_{j}^{\text{dim}(\boldsymbol{\phi})}(1-Q_{\boldsymbol{\phi}_K}(s_j\leq0))\\
%        & \mathbf{z}_k \sim q_{\boldsymbol{\phi}_k};\ \ [\boldsymbol{\phi}_k,\boldsymbol{\zeta}_k] = [\boldsymbol{\phi}_{k-1},\boldsymbol{\zeta}_{k-1}] - [\alpha^{\phi},\alpha^{\zeta}]\nabla_{[\phi,\zeta]} \mathcal{L}_{\mathcal{T}_i^s}(f_{\boldsymbol{\theta}_0 + \boldsymbol{\zeta}_{k-1}\odot\mathbf{z}_{k-1}}).\nonumber
% \end{align}

% Since $\theta_0$ is \emph{fixed} during meta-training,  no significant computation and memory overhead occur; and since $\boldsymbol{\zeta}\odot\mathbf{z}$ is sparse throughout the inner-loops, stitching incur only small changes to the original pre-trained initialization which preserves transferable information. Furthermore, involving the stitched model directly in meta-training also relax the requirement on finding the optimal weighted coefficient for model ensemble. \par

\textbf{Meta-learning mask selection through a hypernetwork.}$\ \ $
%To achieve selective merging of sparse modulation in a task-dependent manner, 
We resort to meta-learning a hypernetwork \js{cite hypernetwork paper} $h_{\boldsymbol{\zeta}}$ for a direct estimation of the mask selection scores $\boldsymbol{\alpha}_i$ in Eqn.~(\ref{eq:smat_constraint_op}), where $\boldsymbol{\alpha}_i$ is conditioned on the task support set $\gT_i^s$. Specifically, we employ the pre-trained model $f_{\theta_{pre}}$ to encode each support set image $\mathbf{x}_{i,j}^s\in\mathcal{T}_i^s$ into a vector embedding $f_{\theta_{pre}}(\mathbf{x}_{i,j}^s)$ at the output of its last layer, before aggregating into class prototypes. We concatenate the prototypes into a sequence as input and feed it into a single trainable transformer block to acquire $\boldsymbol{\alpha}'\in\mathbb{R}^{|\gM|}$ at the output, which we treat as the logits for activating each mask. Finally, we use the Gumbel-Sigmoid trick~\cite{jang2017categorical} for sampling binary activations for the masks followed by normalization to obtain $\boldsymbol{\alpha}\in[0,1]^{|\mathcal{M}|}$. The hypernetwork is meta-trained in an end-to-end fashion following the objective in Eqn.~(\ref{eq:smat_constraint_op}).\par
%%TODO:  why not using a high-way selection, i.e., the selection of mask in the current layer depends on the previous one????

\textbf{Improving mask specialization through dense target bootstrapping.}$\ \ $Having a sparsity penalty on the modulation parameters may impose a more difficult optimization problem in the meta-objective due to the tradeoff with few-shot prediction performance. To compensate for this as well as to further encourage cooperation between sparse modulation upon merging, we take inspiration from bootstrapped meta-learning literature~\cite{flennerhag2022bootstrapped,tack2022selfimproving} and introduce a consistency loss $\mathcal{L}^{bt}_{\mathcal{T}_i^q}(\theta_{i},\theta_{i}^{\mathtt{target}})$ in the meta-objective during meta-tuning, where $\theta_{i}^{\mathtt{target}}$ is a target model derived from the task query set, $\mathcal{T}_i^q$. We reach $\theta_{i}^{\mathtt{target}}$ by taking $K$-step of gradient descent starting from $\theta_i$ on $\mathcal{L}^{ce}_{\mathcal{T}_i^q}$; however, more interestingly, unlike $\theta_i$, we do not restrict the capacity of $\theta_{i}^{\mathtt{target}}$ through sparse regularization which leads to a final $\theta_{i}^{\mathtt{target}}$ that is both dense in modulation i.e., $\theta_{i}^{\mathtt{target}}-\theta_{pre}$ and highly task-specific. Choosing $\mathcal{L}^{bt}_{\mathcal{T}_i^q}$ as the KL-divergence with temperature $\tau$ effectively
%When choosing $\pi$ as a KL-divergence with temperature $\tau$, the matching loss effectively 
encourages knowledge transfer from the dense target at full expressive to the sparsely modulated $\theta_i$, potentially leading to more specialized sparse modulation with improved prediction performance. Of note, we do not backpropagate loss gradients through $\theta_{i}^{\mathtt{target}}$~\cite{flennerhag2022bootstrapped}.\par


\textbf{Meta-optimization with controlled mask sparsity}.$\ \ $We are \chen{now} ready to state ours optimization problem for meta-tuning. Since the sparsity level in modulation is crucial for model capacity and generalization performance~(see~\cref{sec: motivating_example}), it is, therefore, desirable to enable precise \emph{control} of the mask sparsity levels in our meta-tuning algorithm. This can be naturally formulated into a constrained optimization problem
\begin{align}\label{eq:smat_constraint_op}
       \minimize\limits_{\boldsymbol{\theta_\delta},\boldsymbol{\zeta}, \boldsymbol{\Phi}}\ \ \ \ \ \ &\mathbb{E}_{\gT_i\sim p^{\text{train}}(\gT)}\big[\gL^{ce}_{\mathcal{T}_i^q}(\boldsymbol{\theta}_i) + \gL^{bt}_{\gT_i^q}(\theta_i,\theta_{i}^{\mathtt{target}})\big],\nonumber \\
       &\boldsymbol{\theta}_i = \boldsymbol{\theta}_{pre} +  \boldsymbol{\theta}_{\delta}\odot\sum_{m}^{|\gM|}\alpha_{i,m}\boldsymbol{z}_m, \nonumber\\ 
       &\boldsymbol{z}_m\sim q_{\phi_m}; \boldsymbol{\alpha}_i\sim h_{\zeta},\nonumber\\
       % & \mathbf{z}_k \sim q_{\boldsymbol{\phi}_k};\ \ [\boldsymbol{\phi}_k,\boldsymbol{\zeta}_k] = [\boldsymbol{\phi}_{k-1},\boldsymbol{\zeta}_{k-1}] - [\alpha^{\phi},\alpha^{\zeta}]\nabla_{[\phi,\zeta]} \mathcal{L}_{\mathcal{T}_i^s}(f_{\boldsymbol{\theta}_0 + \boldsymbol{\zeta}_{k-1}\odot\mathbf{z}_{k-1}}),\nonumber\\
       \text{subject to }\ \ \ \ \ &\frac{1}{|\boldsymbol{\phi}_m|}\sum_{k}^{|\boldsymbol{\phi}_m|}(1-Q_{\boldsymbol{\phi}_m}(s_k\leq0))\leq\tau_m, \nonumber\\
       &\forall m\in\big[ |\gM| \big],
\end{align}
where $\tau_m\in[0,1]$ are the targeted sparsity levels.
%sparsity in $z_m$ is induced through constraints instead of a penalty in the meta-objective. 
We note that the sparsity constraints are on individual masks as opposed to the overall $\theta_i$ to allow task-dependent sparsity in $\theta_i$ through selective mask merging. For simplicity, we set a common sparsity constraint for all masks i.e., $\tau_m=\tau, \forall m$. This, in turn, implicitly sets the sparsity of $\delta_i$ upon merging to at least $\max(0,1-|\gM|(1-\tau))$.
%\textbf{(b)} only  mask is essential for specialization and the effectiveness in mask merging. Nevertheless, this gives a means to define the minimum overall model sparsity. 
%In practice, we find $\theta_i$ is often sparse in modulation due to sparsity in task-specific mask selection $\mathbf{\alpha}_i$. 
In practice, we optimize the Lagrangian associate with the objective above, i.e., 
\begin{align}\label{eq:smat_unconstraint_op}
    %\boldsymbol{\theta}_\delta^*, \boldsymbol{\zeta}^*, \boldsymbol{\Phi}^*, \boldsymbol{\lambda}^* \notag
    \min\limits_{\boldsymbol{\theta}_\delta, \boldsymbol{\zeta}, \boldsymbol{\Phi}} \max\limits_{\boldsymbol{\lambda}}\ &\mathbb{E}_{\gT_i\sim p^{\text{train}}(\gT)}\big[\gL^{ce}_{\mathcal{T}_i^q}(\boldsymbol{\theta}_i) + \gL^{bt}_{\gT_i^q}(\theta_i,\theta_{i}^{\mathtt{target}})\big] \nonumber \\
    &+ \sum_{m}^{|\gM|}(\frac{\lambda_m}{|\boldsymbol{\phi_m}|}\sum_{k}^{|\boldsymbol{\phi_m}|}(1-Q_{\phi_m}(s_k \leq 0))-\tau)
    % & \mathbf{z}_k \sim q_{\phi_k}; \; [\phi_k, \zeta_k] \leftarrow [\phi_{k-1}, \zeta_{k-1}] \notag \\
    % & \quad\quad\quad - [\alpha^{\phi}, \alpha^{\zeta}] \nabla_{[\phi, \zeta]} \mathcal{L}_{\mathcal{T}_i^s}(f_{\theta_0 + \zeta_{k-1} \odot z_{k-1}}). \nonumber
\end{align}
We resort to simultaneous gradient descent and projected gradient ascent~\cite{gallego-posada2022controlled} for optimizing Eqn.~(\ref{eq:smat_unconstraint_op}). The pseudocodes for meta-training can be found in Appendix~\ref{app:pcode}.
%In practice, due to the sparse and infrequent activation of masks during meta-training, we heuristically scale the learning rate for the Lagrangian multiplier for each mask by $\alpha_i$, thus dynamically avoid over-weighting the sparsity penalty over the performance objective. \par

\subsection{Meta-testing time adaptation}\label{sec: mt_adapt}

\textbf{Gradient-free adaptation.}$\ \ $Prior work has discovered that further task-specific adaptation of a meta-trained model is essential for improving its performance on OOD tasks during meta-testing~\cite{hu2022pmf, chen2023secure, li2022TaskSpecificAdapter}. Although effective, one major limitation of these adaptation methods is the reliance on back-propagation of the gradients which can be expensive, making these methods inefficient and highly impractical due to poor scaling with model size. To this end, we propose an adaptation strategy, specifically designed for SMAT, that bypasses the gradient computation. At the core of our method lies the empirical observation that .... Specifically, we conduct a few rounds of Gibb's sampling to optimize the mask selection scores in a binary search space by minimizing the resultant cross-entropy loss on the support set. We note that the whole process only requires evaluating the support loss but not its gradients. A more detailed description of the algorithm can be found in Appendix~\chen{X}.\par

% Our solution is centered around two of our key empirical observations: (a) there exits a decent mask combination  i.e., better than which is essentially estimated by the hypernetwork, even when restricting mask selection score in a binary search space, i.e., $\in\{0,1\}^{|\mathcal{M}|}$. (b) the optimally of the binary mask combination is seemly proportional to the negative support loss. Remarkably, the evidence suggests that a better test-time solution can already be achieved by adjusting the mask selection scores in binary! It is now intuitively easy to give out our solution which is fully described in Alg.~\ref{alg:foward_mask_score_adaptation}. We conduct a few rounds of Gibb's sampling to optimize the mask selection scores in a binary search space by minimizing its performance on the support set. We note that the whole process only requires evaluating the support loss but not its gradients.\par\par

\textbf{Gradient-based adaptation.}$\ \ $Following~\cite{hu2022pmf}, we also consider gradient-based fine-tuning of our meta-tuned model at meta-testing time. With only few changes, our method is fully compatible with existing full fine-tuning (i.e., fine-tuning the entire model), and existing parameter-efficient fine-tuning~(PEFT) techniques. Specifically, we simply use $\theta_i$ in Eqn.~(\ref{eq:smat_constraint_op}) as the model initialization, before applying any off-the-self fine-tuning technique for adaptation on the support set of each task. 

%pecifically, we first collapse the masks selected by the hypernetwork for a given testing task $\mathcal{T}^{*}$ into $\Theta$ which has the same dimension as the original pre-trained model, then we resort to any particular off-the-shelf PEFT method for gradient-based fine-tuning. In addition, we also consider simply fine-tuning only the un-masked parameters which are specific to each task. Our motivation is that the 









==> tables/average_with_adaptation.tex <==
\begin{table}[t] 
  \centering
\begin{minipage}{0.62\linewidth}
   \caption{Classification accuracy of DomainNet 20-way-1-shot classification tasks.}
   \resizebox{1\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \multirow{2}{*}{\textbf{DomainNet}} & \multicolumn{5}{c}{\textbf{OOD Domains}}\\%&\multicolumn{5}{c}{\textbf{S$\rightarrow$Q Domain Shift}}\\
    \cmidrule(lr){2-6}%\cmidrule(l){7-11}
    &\textbf{S}ketch & \textbf{R}eal  & \textbf{I}nfograph &  \textbf{C}lipart &  \textbf{P}ainting \\ %& S$\rightarrow$R &  R$\rightarrow$I& I$\rightarrow$C  & C$\rightarrow$P &P$\rightarrow$S \\
    \cmidrule(r){1-1} \cmidrule(lr){2-6}%\cmidrule(l){7-11}
    \textbf{\chen{Full}} & $\bm{38.97}\scriptstyle\pm1.15$ & $69.39\scriptstyle\pm1.29$  & $20.89\scriptstyle\pm0.85$ &  $45.33\scriptstyle\pm1.06$ &  $47.37\scriptstyle\pm1.32$ \\
    %& $40.97\scriptstyle\pm1.68$ &  $22.11\scriptstyle\pm0.87$ & $19.19\scriptstyle\pm0.94$  & $34.27\scriptstyle\pm1.16$ &$25.65\scriptstyle\pm0.97$ \\
    \textbf{LoRA} & $38.25\scriptstyle\pm1.13$ & $69.54\scriptstyle\pm1.30$  & $\underline{22.22}\scriptstyle\pm0.87$ &  $\underline{46.25}\scriptstyle\pm1.10$ &  $47.27\scriptstyle\pm1.28$\\
    %& $40.61\scriptstyle\pm1.66$ &  $22.52\scriptstyle\pm0.85$ & $19.55\scriptstyle\pm0.71$  & $34.53\scriptstyle\pm1.24$ &$25.90\scriptstyle\pm0.96$ \\
    \textbf{PMF-IN} & $38.64\scriptstyle\pm1.16$ & $\underline{70.03}\scriptstyle\pm1.33$  & $21.30\scriptstyle\pm0.87$ &  $45.72\scriptstyle\pm1.08$ &  $\underline{48.30}\scriptstyle\pm1.34$ \\
    %& $41.62\scriptstyle\pm1.66$ &  $22.28\scriptstyle\pm0.84$ & $19.20\scriptstyle\pm0.96$  & $34.31\scriptstyle\pm1.23$ &$25.85\scriptstyle\pm0.98$ \\
   \textbf{PMF-MD} & $34.35\scriptstyle\pm1.00$ & $67.43\scriptstyle\pm1.35$  & $19.10\scriptstyle\pm0.89$ &  $42.89\scriptstyle\pm1.14$ &  $43.17\scriptstyle\pm1.41$ \\
   %& $36.72\scriptstyle\pm1.61$ &  $21.79\scriptstyle\pm0.93$ & $18.10\scriptstyle\pm0.96$  & $29.62\scriptstyle\pm1.16$ &$23.65\scriptstyle\pm1.02$ \\
    \cmidrule(r){1-1} \cmidrule(lr){2-6}%\cmidrule(l){7-11}
    \textbf{Ours-IN} & $\underline{38.96}\scriptstyle\pm1.14$ & $\bm{70.43}\scriptstyle\pm1.30$  & $\bm{22.59}\scriptstyle\pm0.91$ &  $\bm{47.58}\scriptstyle\pm1.06$ &  $\bm{49.02}\scriptstyle\pm1.32$ \\
    %& $\bm{41.82}\scriptstyle\pm1.66$ &  $\bm{23.35}\scriptstyle\pm0.88$ & $\bm{20.53}\scriptstyle\pm1.03$  & $\bm{35.68}\scriptstyle\pm1.19$ &$\bm{26.83}\scriptstyle\pm1.02$ \\
     \textbf{Ours-MD} &$\bm{35.51}\scriptstyle\pm1.07$ & $69.76\scriptstyle\pm1.34$  & $20.31\scriptstyle\pm0.84$ &  $42.66\scriptstyle\pm1.22$ &  $43.33\scriptstyle\pm1.38$ \\
     %& $0.1\scriptstyle\pm0.1$ &  $0.1\scriptstyle\pm0.1$ & $0.1\scriptstyle\pm0.1$  & $0.1\scriptstyle\pm0.1$ &$0.1\scriptstyle\pm0.1$ \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:20way1shot-shot-domainnet}
\end{minipage}
\hspace{0.008\linewidth}
\begin{minipage}{0.35\linewidth}
   \caption{Average testing accuracy by class, task and domain-transfer.}
   \resizebox{1\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{}} & \multicolumn{4}{c}{\textbf{Average}}\\%&\multicolumn{5}{c}{\textbf{S$\rightarrow$Q Domain Shift}}\\
    \cmidrule(lr){2-5}%\cmidrule(l){7-11}
    &\cellcolor{DarkGray}\textbf{Class} & \cellcolor{Gray}\textbf{Task}  & \textbf{Domain} &  \textbf{All} \\ %& S$\rightarrow$R &  R$\rightarrow$I& I$\rightarrow$C  & C$\rightarrow$P &P$\rightarrow$S \\
    \cmidrule(r){1-1} \cmidrule(lr){2-5}%\cmidrule(l){7-11}
    \textbf{\chen{Full}} & 
    \cellcolor{DarkGray}$76.91$& 
    \cellcolor{Gray}$74.16$&
    $44.39$ &  
    $65.71$ \\
    \textbf{LoRA} & 
    \cellcolor{DarkGray}$78.96$ &
    \cellcolor{Gray}$74.73$  &
    $44.71$ &  
    $66.98$ \\
    \textbf{PMF-IN} & 
    \cellcolor{DarkGray}$75.90$ &
    \cellcolor{Gray}$76.86$  &
    $44.80$ & 
    $66.11$\\
   \textbf{PMF-MD} &
   \cellcolor{DarkGray}$84.61$ &
   \cellcolor{Gray}$73.17$  &
   $41.39$ &  
   $68.68$ \\
    \cmidrule(r){1-1} \cmidrule(lr){2-5}%\cmidrule(l){7-11}
    \textbf{Ours-IN} & 
    \cellcolor{DarkGray}$76.64$ &
    \cellcolor{Gray}$78.53$ &
    $45.72$ & 
    $67.46$\\
     \textbf{Ours-MD} &
     \cellcolor{DarkGray}$85.26$ &
     \cellcolor{Gray}$73.31$  & 
     $42.31$& 
     $69.35$ \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:meta-tuned_avg_results}
\end{minipage}
\end{table}%

==> tables/curriculum_online.tex <==
\begin{table*}[t]
\caption{Cumulative online accuracy (\%) on the Omniglot-MNIST-FashionMNIST online learning benchmark where tasks are switched with a probability of $1-p$. Reported results are averaged over five trials, subscripts denote the standard deviation, and bold denotes the best result of each group.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
    \toprule
    & \multicolumn{4}{c}{$p=0.98$} & \multicolumn{4}{c}{$p=0.90$} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    Method & Total & Omniglot & MNIST & Fashion & Total & Omniglot & MNIST & Fashion  \\ 
    \midrule
        Online ADAM & 73.9\std{2.2} & 81.7\std{2.3} & 70.0\std{3.6} & 62.3\std{2.5} & 23.8\std{1.2} & 26.6\std{2.0} & 20.0\std{1.4} & 22.1\std{1.3} \\
        Fine Tuning & 72.7\std{1.7} & 80.8\std{2.0} & 68.7\std{2.8} & 59.6\std{3.1} & 22.1\std{1.1} & 25.5\std{1.5} & 18.1\std{1.9} & 19.2\std{1.6} \\
        MAML & 84.5\std{1.7} & 97.3\std{0.3} & 80.4\std{0.3} & 63.5\std{0.3} & 75.5\std{0.7} & 88.8\std{0.4} & 68.1\std{0.5} & 56.2\std{0.4} \\
        ANIL & 75.3\std{2.0} & 95.1\std{0.6} & 58.7\std{2.9} & 49.7\std{0.3} & 69.1\std{0.8} & 88.3\std{0.5} & 52.4\std{0.6} & 47.6\std{0.9} \\
        BGD & 87.8\std{1.3} & 95.1\std{0.5} & 86.9\std{1.1} & 74.4\std{1.1} & 63.4\std{0.9} & 72.8\std{1.2} & 55.9\std{2.2} & 51.7\std{1.3} \\
        MetaCOG & 88.0\std{1.0} & 95.2\std{0.5} & 87.1\std{1.5} & 74.3\std{1.5} & 63.6\std{0.9} & 73.5\std{1.3} & 55.9\std{1.8} & 51.7\std{1.4} \\
        MetaBGD  & 91.1\std{2.6} & 96.8\std{1.5} & 92.5\std{1.9} & 77.8\std{3.8} & 74.8\std{1.1} & 83.1\std{1.0} & 71.7\std{1.5} & 61.5\std{1.2} \\
        Continual MAML  &  92.8\std{0.6} &  \textbf{97.8\std{0.2}} & 93.9\std{0.8} & 79.9\std{0.7} & 83.3\std{0.4} & 89.0\std{0.5} & 84.5\std{0.7} & 71.1\std{0.7} \\
        \textbf{+ SMAT (ours)} & \textbf{93.3\std{0.7}} & 97.5\std{0.4} & \textbf{94.4\std{0.7}} & \textbf{81.5\std{0.8}} & \textbf{85.5\std{0.7}} & \textbf{89.2\std{0.6}} & \textbf{86.4\std{0.8}} & \textbf{74.6\std{0.6}} \\
    \bottomrule
    \end{tabular}
  }
\label{tab:omniglot}
\end{table*}


==> tables/md_without_adaptation.tex <==
\begin{table*}[t] 
  \centering
   \caption{Variable-way-variable-shot classification results \emph{without gradient-based fine-tuning during meta-testing time} for ID and OOD tasks in Meta-dataset. $^\dagger$ and $^\ddagger$ respectively indicate results reported in \cite{hu2022pmf} and \cite{basustrong2023}. \chen{I made new tables in the appendix which might be too big to fir in the main text?, I will keep updating those ones and decide later whehter to include them in the main text.}}
   \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Meta-dataset}} &\textbf{ImageNet} & \textbf{Aircraft}  & \textbf{Omniglot} &  \textbf{CUB} &  \textbf{DTD} & \textbf{QuickDraw} &  \textbf{Fungi}& \textbf{VGGFlower}  & \textbf{TrafficSign} & \textbf{MSCOCO} \\
    \cmidrule(lr){2-11}
    &\multicolumn{8}{c}{\cellcolor{DarkGray}\textbf{IID Domains}}&\multicolumn{2}{c}{\cellcolor{Gray}\textbf{OOD Domains}}\\
    \cmidrule(r){1-1} \cmidrule(lr){2-9}\cmidrule(l){10-11}
    \textbf{$^\ddagger$\chen{Full}} &
    \cellcolor{DarkGray}$73.54\scriptstyle\pm1.15$ &
    \cellcolor{DarkGray}$75.4\scriptstyle\pm1.29$ &
    \cellcolor{DarkGray}$78.7\scriptstyle\pm0.85$ & 
    \cellcolor{DarkGray} $85.4\scriptstyle\pm0.097$ & 
    \cellcolor{DarkGray} $86.9\scriptstyle\pm0.59$ &
    \cellcolor{DarkGray} $73.6\scriptstyle\pm0.71$ &
    \cellcolor{DarkGray} $54.7\scriptstyle\pm0.96$ &
    \cellcolor{DarkGray} $94.2\scriptstyle\pm0.54$  & 
    \cellcolor{Gray}$87.3\scriptstyle\pm0.88$ &
    \cellcolor{Gray}$61.5\scriptstyle\pm0.89$ \\
    \textbf{$^\ddagger$\chen{LoRA}} & 
    \cellcolor{DarkGray}$74.22\scriptstyle\pm2.03$ &
    \cellcolor{DarkGray}$80.8\scriptstyle\pm2.69$  & 
    \cellcolor{DarkGray}$80.8\scriptstyle\pm3.96$ & 
    \cellcolor{DarkGray} $85.8\scriptstyle\pm2.18$ & 
    \cellcolor{DarkGray} $86.8 \scriptstyle\pm1.14$ &
    \cellcolor{DarkGray} $72.7\scriptstyle\pm2.51$ &
    \cellcolor{DarkGray}  $59.8\scriptstyle\pm2.88$ &
    \cellcolor{DarkGray} $94.8\scriptstyle\pm1.44$  & 
    \cellcolor{Gray}$88.1\scriptstyle\pm3.40$ &
    \cellcolor{Gray}$62.1\scriptstyle\pm2.52$ \\
   \textbf{\chen{$^\dagger$PMF-MD (DINO ViT/S)}} &  
   \cellcolor{DarkGray}$74.59\scriptstyle\pm2.07$ &
   \cellcolor{DarkGray}$88.33\scriptstyle\pm1.18$  & 
   \cellcolor{DarkGray}$91.79\scriptstyle\pm1.65$ & 
   \cellcolor{DarkGray}$91.02\scriptstyle\pm1.18$ & 
   \cellcolor{DarkGray}$86.61\scriptstyle\pm1.65$ &
   \cellcolor{DarkGray}$79.23\scriptstyle\pm1.97$ &
   \cellcolor{DarkGray}$74.2\scriptstyle\pm2.21$ &
   \cellcolor{DarkGray}$94.12\scriptstyle\pm1.39$  &
   \cellcolor{Gray}$88.85\scriptstyle\pm3.45$ &
   \cellcolor{Gray}$62.59\scriptstyle\pm2.55$ \\
    \cmidrule(r){1-1} \cmidrule(lr){2-9}\cmidrule(l){10-11}
     \textbf{Ours-MD} & \cellcolor{DarkGray}$73.78\scriptstyle\pm1.15$ &
     \cellcolor{DarkGray}$91.04\scriptstyle\pm1.29$  &
     \cellcolor{DarkGray}$88.84\scriptstyle\pm0.85$ &
     \cellcolor{DarkGray} $91.27\scriptstyle\pm1.06$ &
     \cellcolor{DarkGray} $87.51\scriptstyle\pm1.32$ &
     \cellcolor{DarkGray} $78.94\scriptstyle\pm1.68$ &
     \cellcolor{DarkGray}  $75.95\scriptstyle\pm0.87$ &
     \cellcolor{DarkGray} $94.72\scriptstyle\pm0.94$  & 
     \cellcolor{Gray}$87.09\scriptstyle\pm1.16$ &
     \cellcolor{Gray}$59.52\scriptstyle\pm0.97$ \\
    \cmidrule{1-11}
    & \multicolumn{1}{c}{\cellcolor{DarkGray}\textbf{IID Domains}}&\multicolumn{9}{c}{\cellcolor{Gray}\textbf{OOD Domains}}\\
    \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-11}
    \textbf{\chen{$^\dagger$PMF-IN (DINO ViT/S)}} & 
    \cellcolor{DarkGray}$74.69\scriptstyle\pm1.91$ & 
    \cellcolor{Gray}$76.78\scriptstyle\pm2.75$  &
    \cellcolor{Gray}$80.68\scriptstyle\pm4.10$ &  
    \cellcolor{Gray}$85.04\scriptstyle\pm2.36$ &  
    \cellcolor{Gray}$86.63\scriptstyle\pm1.24$ & 
    \cellcolor{Gray}$71.25\scriptstyle\pm2.71$ &  
    \cellcolor{Gray}$54.78\scriptstyle\pm2.91$ & 
    \cellcolor{Gray}$94.57\scriptstyle\pm1.52$  & 
    \cellcolor{Gray}$88.33\scriptstyle\pm3.43$ &
    \cellcolor{Gray}$62.57\scriptstyle\pm2.46$ \\
    \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-11}
    \textbf{Ours-IN} & 
    \cellcolor{DarkGray}$76.43\scriptstyle\pm2.13$ & 
    \cellcolor{Gray}$82.07\scriptstyle\pm2.97$  &
    \cellcolor{Gray}$71.12\scriptstyle\pm3.9$ &
    \cellcolor{Gray}$87.16\scriptstyle\pm2.23$ & 
    \cellcolor{Gray}$88.45\scriptstyle\pm1.22$ &
    \cellcolor{Gray}$72.58\scriptstyle\pm2.63$ & 
    \cellcolor{Gray}$61.33\scriptstyle\pm2.87$ & 
    \cellcolor{Gray}$95.76\scriptstyle\pm1.35$  &
    \cellcolor{Gray}$85.29\scriptstyle\pm3.31$&
    \cellcolor{Gray}$63.04\scriptstyle\pm2.39$ \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:md_withou_adaptation}
\end{table*}%

==> tables/mnist_online.tex <==
\begin{table}[t]
\centering
  \caption{Retained accuracy (RA) and forward-transfer (FT) for three different MNIST continual learning problems: rotations, permutations and many permutations. Reported results are averaged over three trials, subscripts denote the standard deviation, and bold denotes the best result.}
  \small\centering
  \label{tab:mnist}
   \begin{tabular}{l ll ll ll}
    \toprule
    & \multicolumn{2}{c}{Rotations} & \multicolumn{2}{c}{Permutations} & \multicolumn{2}{c}{Many Permutations} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    & RA ($\uparrow$) & FT ($\uparrow$) & RA ($\uparrow$) & FT ($\uparrow$) & RA ($\uparrow$) & FT ($\uparrow$) \\
    \midrule
    C-MAML & 77.05\std{0.70} & 47.95\std{0.92} & 72.10\std{0.60}& -0.34\std{0.62} & 44.23\std{0.69}&  1.85\std{0.63} \\ 
    La-MAML & 76.57\std{0.79} & 47.87\std{0.98} & 73.66\std{0.46}& -0.19\std{0.55}  & 49.32\std{0.86}& 0.99\std{0.62} \\
    \textbf{+ SMAT (ours)} & \textbf{77.21\std{0.91}}& \textbf{50.36\std{0.88}} & \textbf{77.05\std{0.32}}& \textbf{-0.11\std{0.45}} & \textbf{51.66\std{0.60}}& \textbf{2.44\std{0.49}} \\ 
    \bottomrule
  \end{tabular}
\end{table}
